Galactic Center constraints on self-interacting sterile neutrinos from fermionic dark matter ("ino") models

The neutrino minimal standard model ($\nu$MSM) has been tightly constrained in the recent years, either from dark matter (DM) production or from X-ray and small-scale observations. However, current bounds on sterile neutrino DM can be significantly modified when considering a $\nu$MSM extension, in which the DM candidates interact via a massive (axial) vector field. In particular, standard production mechanisms in the early Universe can be affected through the decay of such a massive mediator. We perform an indirect detection analysis to study how the $\nu$MSM parameter-space constraints are affected by said interactions. We compute the X-ray fluxes considering a DM profile that self-consistently accounts for the particle physics model by using an updated version of the Ruffini-Arg\"uelles-Rueda (RAR) fermionic ("ino") model, instead of phenomenological profiles such as the Navarro-Frenk-White (NFW) distribution. We show that the RAR profile accounting for interacting DM, is compatible with measurements of the Galaxy rotation curve and constraints on the DM self-interacting cross section from the Bullet cluster. A new analysis of the X-ray NuSTAR data in the central parsec of the Milky Way, is here performed to derive constraints on the self-interacting sterile neutrino parameter-space. Such constraints are stronger than those obtained with commonly used DM profiles, due to the dense DM core characteristic of the RAR profiles.

==> figure/RARpBH/figure.tex <==
%\begin{figure}
	%\centering
	%\includegraphics[width=0.77\hsize,clip]{\ROOTPATH/rho.pdf}\\
	%\includegraphics[width=0.77\hsize,clip]{\ROOTPATH/vrot.pdf}
	%\caption{(Color online) Theoretical density profiles and rotation curves of the RAR model with a central BH. The radial window is from the ISCO radius (e.g. 3 Schwarzschild radii of a $\SI{4.2E6}{\Msun}$ BH) all the way to $\SI{E5}{\parsec}$. The gray-black striped curve represents the contribution of the BH only while the DM contributions are labeled with their fermion mass in the $mc^2\sim\si{\kilo\eV}$ region: $\SI{1}{\kilo\eV}$ (dash), $\SI{7}{\kilo\eV}$ (dot-dash) and $\SI{30}{\kilo\eV}$ (solid) with corresponding free RAR model parameters ($\beta_0$,$\theta_0$,$W_0$) in the legend reading for central temperature, degeneracy, and escape parameters respectively. Shown is also the total rotation curve (red thick curve) including the total baryonic (bulge + disk) component.}
	%\label{fig:RARpBH}
%\end{figure

\begin{figure}
	\centering
	\includegraphics[width=0.9\hsize,clip]{\ROOTPATH/rho.pdf}
	\caption{(Color online) Theoretical density profiles of the RAR model with a central BH. The radial window is from the ISCO radius (e.g. 3 Schwarzschild radii of a $\SI{4.2E6}{\Msun}$ BH) all the way to $\SI{E5}{\parsec}$. Each curve is labeled with the corresponding fermion mass in the $mc^2\sim\si{\kilo\eV}$ region: $\SI{1}{\kilo\eV}$ (dash), $\SI{7}{\kilo\eV}$ (dot-dash) and $\SI{30}{\kilo\eV}$ (solid) with corresponding free RAR model parameters ($\beta_0$,$\theta_0$,$W_0$) in the legend reading for central temperature, degeneracy, and escape parameters respectively.}
	\label{fig:RARpBH-rho}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.77\hsize,clip]{\ROOTPATH/vrot.pdf}
	\caption{(Color online) Theoretical rotation curves of the RAR model with a central BH. The radial window is from the ISCO radius (e.g. 3 Schwarzschild radii of a $\SI{4.2E6}{\Msun}$ BH) all the way to $\SI{E5}{\parsec}$. The gray-black striped curve represents the contribution of the BH only while the DM contributions are labeled with their fermion mass in the $mc^2\sim\si{\kilo\eV}$ region: $\SI{1}{\kilo\eV}$ (dash), $\SI{7}{\kilo\eV}$ (dot-dash) and $\SI{30}{\kilo\eV}$ (solid) with corresponding free RAR model parameters ($\beta_0$,$\theta_0$,$W_0$) as in the figure above. Shown is also the total (DM $+$ baryons) rotation curve (red thick curve) which is only well fitted by particle masses above 3.3 keV as detailed in the text.}
	\label{fig:RARpBH-vrot}
\end{figure}
